Hints for a non-standard Higgs boson from the LHC

We reconsider Higgs boson invisible decays into Dark Matter in the light of recent Higgs searches at the LHC. Present hints in the CMS and ATLAS data favor a non-standard Higgs boson with approximately 50% invisible branching ratio, and mass around 143 GeV. This situation can be realized within the simplest thermal scalar singlet Dark Matter model, predicting a Dark Matter mass around 50 GeV and direct detection cross section just below present bound. The present runs of the Xenon100 and LHC experiments can test this possibility.

==> refanswer.tex <==
----------------------------------------------------------------------
Answers to the Referee A -- LH13495/Raidal
----------------------------------------------------------------------

We have addressed both comments of the Referee. The changes made are the following.

1. We explain in the new version of manuscript that Fig. 1 is obtained by us
by performing a \chi^2 fit of the data presented in [1,2]. We explain this both
in the caption and in the text. References are also added.

2. We included both the LHC and LEP excluded regions on the Fig. 2.
Explanations and references are given.

3. We included several new references.

Following the Referee's suggestion, we transfer our paper from PRL to PRD. 




----------------------------------------------------------------------
Answers to the Referee B -- LH13495/Raidal
----------------------------------------------------------------------

We have addressed all three comments of the Referee. The changes made are the following.

1. We explain in the new version of manuscript that Fig. 1 is obtained by us
by performing a \chi^2 fit of the data presented in [1,2]. We explain this both
in the caption and in the text. References are also added.

2. We explain the experimental situation in more detail in the new version of manuscript.

3. We comment on the results of other direct detection experiments, in particular DAMA, CoGeNT 
and CRESST II and cite papers that perform global fits to all available data. The results of those
papers is that those experiments are consistent with XENON100 only if extremely unlikely assumptions
are made on cosmology and physics. In the model we consider the predictions are under control. 

4. We have added several new references.

Following the Referee's criticism, we transfer our paper from PRL to PRD. 

